Device Sampling and Resource Optimization for Federated Learning in Cooperative Edge Networks

The conventional federated learning (FedL) architecture distributes machine learning (ML) across worker devices by having them train local models that are periodically aggregated by a server. FedL ignores two important characteristics of contemporary wireless networks, however: (i) the network may contain heterogeneous communication/computation resources, and (ii) there may be significant overlaps in devices' local data distributions. In this work, we develop a novel optimization methodology that jointly accounts for these factors via intelligent device sampling complemented by device-to-device (D2D) offloading. Our optimization methodology aims to select the best combination of sampled nodes and data offloading configuration to maximize FedL training accuracy while minimizing data processing and D2D communication resource consumption subject to realistic constraints on the network topology and device capabilities. Theoretical analysis of the D2D offloading subproblem leads to new FedL convergence bounds and an efficient sequential convex optimizer. Using these results, we develop a sampling methodology based on graph convolutional networks (GCNs) which learns the relationship between network attributes, sampled nodes, and D2D data offloading to maximize FedL accuracy. Through evaluation on popular datasets and real-world network measurements from our edge testbed, we find that our methodology outperforms popular device sampling methodologies from literature in terms of ML model performance, data processing overhead, and energy consumption.

==> graveyard.tex <==
graveyard


\begin{algorithm}
\SetAlgoLined
 \textbf{Input} GCN outputs $O$, Adjacency matrix $A$, Device initial data $D(0)$;\\
 \textbf{Output} Sampling scheme $x$ such that $N = \sum_{i=1}^V x_i$;
 \While{$ \sum_{i=1}^V x_i < N$}{
  \eIf{$ \sum_{i=1}^V x_i == 0$}{
   %$i^* = {argmax}_i D_i(0)$ \;
   $x_{{argmax}_i D_i(0)} = 1$\; 
   }{
   %$j^* = {argmin}_j (\cup_{i=1}^{V}x_i\mathcal{D}_i) \cap \mathcal{D}_j$\;
   $x_{{argmin}_j (\cup_{i=1}^{V}x_i\mathcal{D}_i) \cap \mathcal{D}_j} = 1$\;
  }
 }
 \caption{Branch post-processing}
 \label{alg:branch}
\end{algorithm}


\begin{comment}
\begin{table*}[t]
\begin{minipage}{0.99\textwidth}
{\footnotesize
\begin{equation}\label{eq:firstWeightUpdate}
 \widehat{\mathbf{w}}^{(k+1)}_{n'}=\frac{\displaystyle \sum_{j
    \in \mathcal{Q}(n)}|D_j| \mathbf{w}^{(k)}_{j}} {{|\mathcal{Q}(n)|}}-   \frac{\displaystyle \sum_{j
    \in \mathcal{Q}(n)}\beta |D_j|\nabla f_{j}(\mathbf{w}^{(k)}_{j})} {|\mathcal{Q}(n)|}  +\mathbbm{1}^{(k+1)}_{\left\{\mathcal{Q}(n)\right\}}  \mathbf{c}^{(k+1)}_{n'},~~ n'\in \mathcal{Q}(n)
 \end{equation}
 \hrulefill
 \begin{equation}\label{eq:secondWeightUpdate}
  \hspace{-10mm}
 \begin{aligned}
 \widehat{\mathbf{w}}^{(k+1)}_{n'}=&\frac{\displaystyle \sum_{i
    \in \mathcal{Q}(n)} \sum_{j
    \in \mathcal{Q}(i)} |D_j| \mathbf{w}^{(k)}_{j}} {|\mathcal{Q}(n)|} - \frac{\displaystyle \sum_{i
    \in \mathcal{Q}(n)} \sum_{j
    \in \mathcal{Q}(i)} \beta |D_j|\nabla f_{j}(\mathbf{w}^{(k)}_{j})} {|\mathcal{Q}(n)|} + \frac{\displaystyle\sum_{i
    \in \mathcal{Q}(n)}\mathbbm{1}^{(k+1)}_{\left\{{\mathcal{Q}(i)}\right\}}|\mathcal{Q}(i)|  \mathbf{c}^{(k+1)}_{i'}}{|\mathcal{Q}(n)|}+\mathbbm{1}^{(k+1)}_{\left\{\mathcal{Q}(n)\right\}}  \mathbf{c}^{(k+1)}_{n'},~ n'\in Q(n)
     \end{aligned}
     \hspace{-8mm}
 \end{equation}
\hrulefill
}
\end{minipage}
\end{table*}
\end{comment}













\begin{align} \label{eq:sp1}
& \underset{\tilde{s},\tilde{r}}{argmin} %s_{ki},r_{k},r_i
& & \sum_{i \in n} \Bigg(\sum_{j=1}^{|G_i|}p_j + c_{is} + \beta\frac{L(w_i|G_i)|G_i|}{|G_V|}\Bigg) \\ \label{eq:sp2}
& & & + \sum_{k \notin n} D_k \Bigg(\underset{k \neq i}{\sum_{i \in n} }c_{ki}s_{ki} \Bigg) \\
& \text{subject to}
& & \text{Constraints} \ (\ref{eq:con1}-\ref{eq:con4})
\end{align}

Since the constraints (\ref{eq:con1}-\ref{eq:con4}) focus primarily on the offloading and discarding variables, the constraints for (\ref{eq:sp1}-\ref{eq:sp2}) are the same as those for (\ref{eq:obj1}-\ref{eq:obj2}).


\begin{align} \label{eq:sp3}
& \underset{n}{argmin} 
& & \sum_{i \in n} \Bigg(\sum_{j=1}^{|G_i|}p_j + c_{is} + \beta\frac{L(w_i|G_i)|G_i|}{|G_V|}\Bigg) \\ \label{eq:sp4}
& & & + \sum_{k \notin n} D_k \Bigg(\underset{k \neq i}{\sum_{i \in n^*} }c_{ki}s_{ki}\Bigg) \\ 
& \text{subject to}
& & \text{Constraints} \ (\ref{eq:con1}-\ref{eq:con4})
\end{align}

We reformat (\ref{eq:sp1}-\ref{eq:sp2}) by observing its Langrangian and formulating its dual problem as follows:

\begin{align}
& \mathcal{L}(\tilde{s},\tilde{r},\uline{\mu}) =
& & \sum_{i \in n^*} (\sum_j^{|G_i|} p_j + c_is + \beta\frac{L(w_i(T)|G_i)|G_i|}{|G_V|}) \\
& & & + \sum_{k \notin n^*}D_k(\sum_{i \in n^*} c_{ki}s_{ki} + r_k) \\
& & & + \sum_i \mu_i (C_i -\sum_{j}^{|\sum D_ks_{ki}|}c_{ji}) \\
& & & + \sum_i \bar{\mu}_i (P_i - \sum_j^{|G_i|}p_j) \\
& & & + \hat{\mu}(C_s - \sum_{i\in n^*} c_{is})
\end{align}



Solving (\ref{eq:obj1}-\ref{eq:obj2}) can then be done iteratively by alternating solutions between (\ref{eq:sp1}) and (\ref{eq:sp2}).

The resulting algorithm for sampled FedL:
\begin{algorithm}
\SetAlgoLined
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{test}
\Output{test}

initialize \;
 \For{t=0,1..,T}{
  for each node $v_i$ in the sampled set\;
  \eIf{condition}{
   instructions1\;
   instructions2\;
   }{
   instructions3\;
  }
 }
 \caption{Sampled FedL}
\end{algorithm}



\begin{align}
& \underset{n,\tilde{s},\tilde{r}}{\text{argmin}}
& & \sum_{i \in n} \Bigg(\sum_{j=1}^{|G_i|}p_j + c_{is} + \beta\frac{L(w_i|G_i)|G_i|}{|G_V|}\Bigg) \label{eq:obj1} \\ 
& & & + \sum_{k \notin n} D_k \Bigg(\underset{k \neq i}{\sum_{i \in n} }c_{ki}s_{ki}\Bigg) \label{eq:obj2} \\ 
& \text{subject to}
& & G_i = (D_i + \sum_{k \notin n^*}D_ks_{ki})(1-r_i),\ r_i \in [0,1], \label{eq:con1} \\  
& & & \sum_{i \in n} D_ks_{ki}c_{ki} \leq C_k, \sum_{k \notin n} D_ks_{ki} \leq C_i, \label{eq:con2} \\ 
& & & \sum_{i\in n}s_{ki} \leq 1,\ s_{ki} \in \alpha_k \alpha_i [0,1], \ \alpha \in (0,1),  \label{eq:con3} \\ 
& & & \ G_V = \sum_{i \in n} G_i, \ G_ip_{j} \leq P_i, \ \sum_{i\in n} c_{is} \leq C_s, \label{eq:con4}\\ 
& & & x = (x_0,x_1,...,x_{V-1}) \in \{0,1\}^V, \ N = \sum_{i \in V} x_i \label{eq:con5}
\end{align}



{\color{blue}
Some suggestions written by Ali:
\begin{itemize}
    \item The main point we wanna convey across: We are the first who does device sampling considering the inherent network structure for FL.
    \item The edge weight can also describe the tendency of data sharing among the node.
    \item In that way, we have to do the sampling w.r.t. the sharing preference between the devices. (Please take a look at Chris INFOCOM paper).
    \item In this case, you first come up with the optimal set of sampled devices. Then, you can have a mathematical problem formulation regarding the offloading.
    \item The difference between your case and Chris's INFOCOM paper would be in your case, you would have only a limtied set of devices that are designated to communicate to the base stations (say 10 out of 1000) and then given the set, you would need to find the optimal offloading scheme. This makes your problem harder and the studied problem in that INFOCOM a special case of your solution.
    \item Another parameter of interest that you can put in your feature set is link failure probability (probability of failure of communication from a device to a BS). This will change the solution a lot. Also, the rate of communication to the BS can be another factor. In that case, the sampling solution will be different. (Since a pat of this work is experiments, let us make it as general (and non-trivial) as possible.
    \item I can share with you some results on device sampling. Basically the convergence speed of FL upon having device sampling. That would provide an analytical upper bound on the rate of convergence.
    \item Then, you can modify it and put as the objective of the optimization problem and study its characteristics. 
    \item Another idea is adaptive sampling. Assume that I have 1000 devices. You can propose an adaptive algorithm that starts with sampling optimal $10$ and $50$ nodes and see the trade-off between the learning rate and the power consumption, BW usage, etc. Then those two numbers can be adapted until converging to a unique number (e.g., $[10,50] -> [20,35] -> [30,30]$ that you find out that $30$ nodes are the optimal number of nodes considering power consumption, BW usage , etc.)  
    \item Formulating the problem w.r.t the edge weights. In the end, each node will offload its data set to those who has the least similarity, so it will increase the homogeniety of the data.
    \item Model the processing time W.r.t cpu cycles. Consider the size of the transmitted gradient into the offloading part and obtain the number of SGD iterations they can do to have the same offloading time. This also involves heterogeneous computational capabilities.
    \item Edge weight: probablistic similarity. Upon data offloading if a node finds that a very similar set of features exist in its dataset, it will discard it. Then, there would be a discard probability. Then, the problem becomes probabilistic (forming probability distribution of offload among the nodes such as to keep the discarding probability below a threshed, and decreasing the loss)
    \item Periodic sampling--- keep tracking of the optimal set, upon severe changes, change the optimal set upon having stochastic environment. 
\end{itemize}
}




Rearranging:
\begin{align}
&||w_s(t)-v_k(t)|| - (2\eta\beta+1)||w_s(t-1)-v_k(t-1)|| \nonumber \\
& \leq \eta \delta(t-1) ((\eta \beta + 1)^{t-1-(k-1)\tau}-1)
\end{align}
Additionally, as we assume that $\eta \leq \frac{1}{\beta}$,
\begin{align}
&||w_s(t)-v_k(t)|| - (2\eta\beta+1)||w_s(t-1)-v_k(t-1)|| \nonumber \\
& \leq ||w_s(t)-v_k(t)|| - ||w_s(t-1)-v_k(t-1)|| \nonumber \\
& \leq \frac{\delta(t-1)}{\beta} (2^{t-1-(k-1)\tau}-1)
\end{align}
If we represent the previous equation as a telescoping series,
\begin{align}
&\Vert w_s(t)-v_k(t)\Vert \nonumber \\
&= \sum_{y=(k-1)\tau+1}^{t} (||w_s(y)-v_k(y)|| \nonumber \\ 
&- ||w_s(y-1)-v_k(y-1)||) \nonumber \\
& \leq \sum_{y=(k-1)\tau+1}^{t} \frac{\delta(y-1)}{\beta}(2^{y-1-(k-1)\tau}-1) \nonumber \\
& = \frac{1}{\beta} \sum_{y=(k-1)\tau+1}^{t} \Bigg[\frac{\sum_{i=0}^{V-1}x_iD_i(y-1)\delta_i}{\sum_{i=0}^{V-1}x_iD_i(y-1)} (2^{y-1-(k-1)\tau}-1)\Bigg]
\end{align}




where $\gamma_i$

\begin{comment}
&\leq \frac{\gamma_i}{\sqrt{D_i(t)}} + 2(\beta_1 + \beta_2\Vert \nabla L(w_s(t)|\sum_{i=0}^{V-1}x_iD_i(t))) \Vert \nonumber \\
&\leq \frac{\gamma_i}{\sqrt{D_i(t)}} + 2(\beta_1 + 2\beta_2 \rho (L(w_s(t)) - L(w^*))) \nonumber \\
&\leq \frac{\gamma_i}{\sqrt{D_i(t)}} + 2(\beta_1 + 2\beta_2 \rho (\epsilon_0 +\rho h(t)))
\end{comment}




The above analysis was for resource constrained devices which lead to $\sum_{i=0}^{V-1} x_iD_i(t) \neq D_V(t)$. When the network and devices are unconstrained, i.e. $\sum_{i=0}^{V-1} x_iD_i(t) = D_V(t)$, $e_k(w_s(t)) = 0$ and the error convergence
\begin{align}
&\Vert\nabla L(w_s(t)|D_i(t)) - \nabla L(w_s(t)|\sum_{i=0}^{V-1}D_i(t)) - e_k(w_s(t)) \Vert \nonumber \\
&= \Vert\nabla L(w_s(t)|D_i(t)) - \nabla L(w_s(t)|\sum_{i=0}^{V-1}D_i(t)) \Vert \leq \frac{\gamma_i}{\sqrt{D_i(t)}}
\end{align}


\sout{learning consists of image inputs fed} \ali{learning procedure consists of sequential feeding of and input image (or any data defined over an Euclidean space)} into \sout{sequential} \ali{a cascade (or a series) of} 2D convolution layers that map \sout{each pixel neighborhood} \ali{the features of pixels in different neighborhoods} \sout{into a new scaled value} \ali{to different scaled values}. The traditional 2D convolution \ali{used in CNNs} does not apply well \sout{in} \sout{non-euclidean} \ali{where the underlying data is defined over non-Euclidean spaces} \sout{and non-grid domains}, \sout{such as those used to represent network graphs} \ali{e.g., graph structures}. \sout{ Instead,} \ali{Motivated by this fact,} GCNs generalize the 2D convolution into graph convolutions \ali{Citations....} \sout{, a non-euclidean operation that maps a non-grid node neighborhood into a new point}. \sout{In this sense, GCNs are a more general interpretation of CNNs.} The resulting structure of GCNs \sout{then} consists of sequential forward passes through graph convolutional layers, with activation and/or dropout layers in between. Graph convolutions effectively embed network relationships as features, and each subsequent graph convolution layer \sout{develops} \ali{captures} connections \sout{between} \ali{among} \sout{node} \ali{nodes located in different} neighborhoods. Consequently, as the GCN processes \sout{fog network graphs} \ali{a network graph}, it connects features located in ostensibly disconnected subgraphs together \ali{explicitly considering the connections between the nodes}. We include a high-level illustration of feature embedding in the box titled GCN structure in Fig. \ref{fig:gcn_architecture}. GCNs typically output a vector or matrix of probabilities which by itself tends to perform very poorly \cite{li2018combinatorial}. Though their performance in isolation is poor, careful application reveals useful information about the underlying graph relationships \ali{I have no idea what this sentence is trying to say. Careful application?}. 



## PROOF OF THEOREM 2 (OLD)

as in Theorem 1; and $\epsilon_0$ is the positive root of $\frac{1}{f(\epsilon)} = \epsilon$ and is lower bounded by
\begin{align}
&\frac{1}{tw\eta} +\sqrt{\frac{1}{(tw\eta)^2} + \frac{\rho Kh(\tau)+\rho h(t)}{tw\eta/2}}
\end{align}

\begin{proof}
Recall from Theorem 1 above that $||w_s(t)-v_k(t)|| \leq h(t)$ and that  $||L(w_s(t)) - L(v_k(t))|| \leq \rho \Upsilon(t,k) - \Vert e_k(w_s(t))\Vert $. Defining $\theta_k(t) = L(v_k(t))-L(w^*) \geq \epsilon$, and using Theorem 1, we can write:
\begin{align}
&\frac{1}{L(w_s(t))-L(w^*)} - \frac{1}{\theta_{K+1}(t)} \nonumber \\ &=\frac{L(v_{K+1}(t)) - L(w_s(t))}{(L(w_s(t))-L(w^*))\theta_{K+1}(t)} \geq \frac{-\rho h(t)}{\epsilon^2}
\end{align}
and, by using the fact that $\frac{1}{\theta_{K+1}(t)} - \frac{1}{\theta_1(0)} \geq tw\eta(1-\frac{\beta\eta}{2})-K\frac{\rho h(\tau)}{\epsilon^2}$ from Theorem 1 of \cite{tu2020network},
\begin{align}
&\frac{1}{L(w_s(t))-L(w^*)} \leq \frac{1}{f(t)}
\end{align}
where 
\begin{align}
&f(t) =twn(1-\frac{\beta \eta}{2}) -\frac{\rho}{\epsilon^2}(Kh(\tau)+h(t))
\end{align}
Then we can show that either i) $L(w_s(t)) - L(w^*) \leq \epsilon_0$ or ii) $\underset{k\leq K}{min} L(v_k(k\tau)) - L(w^*) \leq \epsilon_0$. And, after applying the triangle inequality,
\begin{align}
&L(w_s(t)) \leq L(v_k(t)) +\rho h(t)
\end{align}
Since $L(v_k(t))\leq L(w^*)+\epsilon_0$, 
\begin{align}
&L(w_s(t)) - L(w^*) \leq  \epsilon_0 +\rho h(t)
\end{align}
\end{proof}



While the objective function (\ref{eq:obj}) appears straightforward, the constraints (\ref{eq:con1}-\ref{eq:con9}) connect the floating point variables $\tilde{s}$ and the integer variables $x$, and make the resulting optimization problem a mixed-integer programming problem as well as a sum-of-ratios fractional programming problem, which is very difficult to solve. Therefore, we decompose the problem in (\ref{eq:obj}) into two interconnected subproblems, and iteratively solve it. The first subproblem solves for $\tilde{s}$ while the second subproblem solves for $x$.

\begin{enumerate}
    \item At time $t=1$, server $s$ calculates the average gradient of the sampled parameters $\nabla \tilde{L}(1)$, then performs the optimization procedure at that time instance. 
    \item While $t \in \{1,...,\tau-1\}$, there is no server-to-device communication or vice versa. As data offloading is occurring at all time instances, $s$ must continue estimating $\nabla \tilde{L}(t) \leftarrow \frac{\nabla \tilde{L}(t-1)}{\alpha_{1}}$ with $\alpha_1 > 1$.
    \item At times $t = k\tau$ for $k \in \{1,...,K \}$, as $s$ receives latest parameters from sampled devices and the true gradients, it aggregates parameters and performs an averaging of the true gradients, obtaining $\nabla \tilde{L}(k\tau)$. At the same time, we must adjust the estimated correction factor $\alpha_{k-1}$ so that it matches what it should have been, i.e. $\alpha_{k} \leftarrow \frac{\nabla \tilde{L}(k\tau-\tau+1) - \nabla \tile{L}(k\tau)}{\tau}$.
    
    [A,B]== B-A+1 =tau
\end{enumerate}

\begin{comment}
\begin{figure}[t]
\includegraphics[width=.45\textwidth]{pix/toy_example.pdf}
\centering
\caption{Toy example with 10 camera-equipped self-driving cars, a server with only 3 available bidirectional links, and 3 objects of interest:  - purple, pants - orange, and hats - green. The number beneath each camera indicates the size of its local dataset, while the robustness of the connecting lines between cameras indicates the strength, security, and bandwidth. Finding an optimal sampling scheme for such a scenario is very challenging.}
\label{fig:toy_ex}
\vspace{-5mm}
\end{figure}
\end{comment}

% For example, the data gathered from the environment by smart cars or cellular mobile devices that are in close proximity, or the information gleaned by UAVs conducting surveillance from the same area are expected to have some degree of similarity. In such cases, using all the data of the users in training can cause model bias toward certain features for specific labels. For instance, in image segmentation scenario, the model can get biased toward detecting a specific tree (e.g., Eastern Cottonwood) that grows in the regions where the majority of the smart cars collect data, which will result in a poor performance of detecting the other kinds of trees. To capture these similarities, we go beyond the star topology of FedL (see Fig.~\ref{fig:simpleFL}) and introduce a network graph among the devices capturing such data similarities. 

% Distributed machine learning is a set of frameworks used to train ML models in a decentralized manner. Devices locally compute gradient descent iterations on their local datasets and transfer the resulting parameters to some network element, which is typically managed by a central server \cite{mcmahan2017communication}. However, in fog environments, the device characteristics are much more diverse and the network conditions are less idealized, featuring imbalanced device datasets and heterogeneous communication links, for example. We focus on federated learning methods over fog networks in particular, which are popular realizations of distributed machine learning noted for their preservation of user privacy and their treatment of diverse non-i.i.d datasets~\cite{hosseinalipour2020federated}.

==> more_exps/optim_complement.tex <==



==> staging_area.tex <==
We assume that the cost of data transmission from devices $\mathcal{V}$ to the server $s$ is homogeneous and that the server-to-device budget is limited to $N$. The state of uplink capabilities is denoted by the binary vector $x$. For example, if device $v_i$ is selected, the corresponding uplink flag $x_i = 1$ and $x_i = 0$ otherwise. 

The number of CPU cycles needed to process a datum at device $v_{i}$ is denoted by $p_i$, and is termed the processing cost. Note that the process cost can be determined offline \cite{miettinen2010energy}, and we assume that it is a constant. Each device has a processing cost limit of $\tilde{C_i}(t)$ indicating the total available cpu cycles. Since the network has both device and server limitations, an optimal sampling procedure to select the best set of devices already has value, especially given that device data distributions are potentially dependent.

However, device $v_i$ may not be attaining its processing cost limit $\tilde{C_i}(t)$. Therefore, we introduce cooperative data sharing between sampled devices (all devices $v_i$ such that $x_i = 1$) and unsampled devices (all devices $v_i$ such that $x_i = 0$), to maximize use of available computational resources. 

We denote the cost per datum of sharing from device $v_k$ to $v_i$ by $c_{ki}$. Note that the data sharing costs are heterogeneous between different combinations of nodes, i.e. $c_{ki}(t) \neq c_{kj}(t)$, and that only unsampled nodes are capable of sharing data. The ratio of data shared between devices $v_i$ and $v_k$ is denoted $s_{ki}$. Since not all of the data needs to be shared, the total ratio of data shared by device $v_k$ can be expressed as $\sum_{i=0}^{V-1} s_{ki}x_{i} \leq 1$. Correspondingly, the total received data $R_i(t)$ at device $v_i$ at time $t$ is expressed as $R_{i}(t) = \sum_{k=0}^{V-1}D_k(t)s_{ki}(t)(1-A_{k,i}(t))(1-x_{k})$. Over time, the weights of the sampled nodes tend to $1$ as their empirical data become less heterogeneous. In addition, all devices that share data are constrained by a sharing cost limit, e.g. $T_k(t)$  for device $v_k$, while receiving devices are limited by their receive buffer capacity, e.g. $R_i(t) \leq C_i(t)$ for device $v_i$. The resulting empirical dataset at node $v_i$ becomes $D_i(t+1) = D_i(t) + R_i(t)$, where $R_i(t)$ denotes the total received data at time $t$. 


\subsubsection{Federated learning constraints} \label{sss:new}
Federated learning has three particular features that reduce the effectiveness of traditional distributed training methods: 1) D2D dependent distributions, 2) extreme device heterogeneity, and 3) limited intra-network communication and coordination resources not only among the set $V$ of devices but also between devices and the server $s$. 

The heterogeneity in regards to device capabilities within federated learning networks hampers model training. For example, each device $v_i$ has a unique capacity for received data $C_i(t)$ and the ratio of total cpu clock cycles and memory devoted to federated learning varies across devices. Combined with the fact that geographically close devices are likely to have partially overlapping datasets ($D_i(t) \cap D_j(t) \notin \{\emptyset\}$), the value derived from tracking, processing, and maintaining all devices within a resource-constrained, federated learning network becomes questionable. 

As mentioned in section \ref{sss:graph}, edge weights indicate the degree to which two connected devices have similar empirical distributions $D_i(t)$ and $D_j(t)$. Application of classic loss averaging methods, i.e. (\ref{eq:Lws}), results in double counting of data $d \in D_i(t) \cap D_j(t)$ when $D_i(t) \cap D_j(t) \notin \{\emptyset\}$. The corresponding loss function in such an environment must take into account possible double counting as in (\ref{eq:newLws}). 

Even with unlimited intra-network communication and coordination resources, the server $s$ would have to have prior knowledge of the exact empirical dataset $D_i(t)$ for all devices $i \in V$ and filter all the resulting loss functions $L(w_i(k\tau)|D_i(k\tau))$ in real time to account for double counting. This becomes even more challenging when we consider the limited communication and coordination resources in typically federated scenarios. Therefore, it is unlikely that the server can coordinate such an intricate procedure. 


We propose smart device sampling with D2D offloading from unsampled nodes $\hat{\mathcal{S}}$ to sampled ones $\mathcal{S}$. By sampling key devices, based on their inherent capabilities and their local dataset, we anchor the network on those select devices so that structured offloading can occur in order to learn a model that can decipher all types of data within the dataset and use stragglers for their valuable local data.

$\boldsymbol{\Phi}(t) \triangleq [\phi_{i,j}]_{1\leq i,j\leq N}$
Explain fixed network assumption that device characteristics are fixed for local iterations, and only change between global aggregations

% Specifically, the loss function $F(\mathbf{w}_i(t-1)|\mathcal{D}_i(t))$ in (\ref{eq:gd}) refers to the average classification error resulting from classifying all $(x_d,y_d) \in \mathcal{D}_i(t)$ using parameters $\mathbf{w}_i(t-1)$, i.e:
% \begin{align}
%     F(\mathbf{w}_i(t-1)|\mathcal{D}_i(t)) = \frac {\sum_{d \in \mathcal{D}_i(t)} f(\mathbf{w}_i(t-1),x_d,y_d)}{\mathcal{D}_i(t)},
% \end{align}
% While the devices apply their local ML model to perform classification tasks in real-time, the network attempts to minimize the global loss induced by the sampled federated parameters $w_s(t)$ on the total unique data within the network 

% The effective received data from $k$ to $i$ is a scaled version of the the raw received data transferred from $k$ to $i$ by the connectivity-similarity factor $1-\Lambda_{k,i}(t)$.  
% since the nodes sample iid from their own datasets (as devices and server cannot know the exact data at other devices they cannot coordinate exact data points to be offloading) for offloading, the server doesn't know the exact number of similar datapoints the other dudes receive. due to htis lack of knowledge, we propose a linear approximation of the connectivity-similarity edge weights where for two nodes k,i if at time t no offloading occurs the edge weights remain unchanged, else the edge weight increases as a function of the ratio of data offloaded from k to i. 

% \ali{
% Since it is difficult to get exact knowledge of underlying device data distributions, we estimate them instead.

%  Since neither the server nor the devices have exact information about the underlying data distributions, we estimate the underlying device to device similarity at connected nodes based on the network application. 
 
% The similarity matrix $\boldsymbol{\Lambda}(t)$ can be not symmetric. As an extreme example, 
 
% picture two devices $i,j$ with $D_i(t) \gg  D_j(t)$, it is possible for $D_j(t) \subseteq D_i(t)$ but not vice versa. We limit similarity measurements to single-hop cases and we assume that the total unique data in the network is fixed, i.e. $D_{\mathcal{N}}$ is a constant.
% }

% So far our problem model has elucidated two clear problems in FedL frameworks: i) extreme device heterogeneity including stragglers and ii) overlapping datasets which will lead to a ML model that is biased towards specific labels of data. 

% We propose a network-aware sampling scheme with optimized D2D offloading to improve classification performance. 



\begin{figure}[!t]
\centering
\includegraphics[width=0.48\textwidth,height=4cm]{pix/prince_ailab.jpg}
\caption{The testbed consists of an assortment of edge and IoT development boards, such as the Jetson Nano, UP3, and Carol TPU.}
\label{fig:testbed}
\end{figure}


\begin{table}[t]
\begin{tabularx}{0.48\textwidth}{c *{3}{Y}}
\toprule[.2em]
\bf{Percentile of} & \multirow{2}{*}{\bf{Smart}} & \multirow{2}{*}{\bf{Random}} & \multirow{2}{*}{\bf{Heuristic}}\\
\bf{FedL accuracy (\%)} &  &  & \\
\midrule
40 &  &  \\
50 &  &  \\
60 & \rule{5 mm}{0.2pt}& \rule{5 mm}{0.2pt} \\
70 &  & \\
\bottomrule
\end{tabularx}

\caption{Comparing the energy consumed to reach baseline levels of FedL accuracy of a CNN trained for Fashion-MNIST dataset for three schemes with offloading. All three schemes attempt to sample 6 devices from a network of 600 devices.}
\label{tab: cost}
%\vspace{-0.2in}
\end{table}

\begin{table}[t]
\begin{tabularx}{0.48\textwidth}{c *{3}{Y}}
\toprule[.2em]
\multirow{2}{*}{\bf{ \% to FedL (\%)}} & \multicolumn{3}{c}{\bf{Cumulative Data Processed}}\\
\cmidrule(lr){2-4}
& \bf{Smart} & \bf{Random} & \bf{Heuristic} \\
\midrule
40 &  &  \\
50 &  &  \\
60 & \rule{5 mm}{0.2pt}& \rule{5 mm}{0.2pt} \\
70 &  & \\
\bottomrule
\end{tabularx}
\end{table}
